PyMT5: multi-mode translation of natural language and Python code with transformers

Simultaneously modeling source code and natural language has many exciting applications in automated software development and understanding. Pursuant to achieving such technology, we introduce PyMT5, the Python method text-to-text transfer transformer, which is trained to translate between all pairs of Python method feature combinations: a single model that can both predict whole methods from natural language documentation strings (docstrings) and summarize code into docstrings of any common style. We present an analysis and modeling effort of a large-scale parallel corpus of 26 million Python methods and 7.7 million method-docstring pairs, demonstrating that for docstring and method generation, PyMT5 outperforms similarly-sized auto-regressive language models (GPT2) which were English pre-trained or randomly initialized. On the CodeSearchNet test set, our best model predicts 92.1% syntactically correct method bodies, achieved a BLEU score of 8.59 for method generation and 16.3 for docstring generation (summarization), and achieved a ROUGE-L F-score of 24.8 for method generation and 36.7 for docstring generation.

==> pre-training-args.tex <==
\begin{figure}[tb]
\begin{minted}[fontsize=\scriptsize]{bash}
TOTAL_NUM_UPDATES=1300000
WARMUP_UPDATES=5000
LR=9.1875e-05
MAX_TOKENS=2200
UPDATE_FREQ=64
DIR=<data-dir>

fairseq-train $DIR$ \
    --max-tokens $MAX_TOKENS \
    --task translation \
    --source-lang src --target-lang tgt \
    --share-all-embeddings \
    --share-decoder-input-output-embed \
    --arch transformer \
    --dropout 0.2 --relu-dropout 0.2 \
    --attention-dropout 0.2 \
    --encoder-embed-dim 1472 \
    --decoder-embed-dim 1472 \
    --max-target-positions 1024 \
    --max-source-positions 1024 \
    --encoder-ffn-embed-dim 4096 \
    --decoder-ffn-embed-dim 4096 \
    --encoder-attention-heads 8 \
    --decoder-attention-heads 8 \
    --criterion label_smoothed_cross_entropy \
    --label-smoothing 0.1 \
    --dropout 0.1 --attention-dropout 0.1 \
    --weight-decay 0.01 --optimizer adam \
    --clip-norm 0.1 \
    --lr-scheduler inverse_sqrt --lr $LR \
    --warmup-updates $WARMUP_UPDATES \
    --update-freq $UPDATE_FREQ \
    --skip-invalid-size-inputs-valid-test \
    --save-dir $DIR/models \
    --save-interval 16 \
    --fp16 --adam-betas '(0.9,0.98)' --adam-eps 1e-6 \
    --tensorboard-logdir $DIR/tensorboard \
    --decoder-learned-pos --encoder-learned-pos
  \end{minted}
  \caption{The \texttt{fairseq-train} script used to  pre-train \ourmodel.}
  \label{fig:pre-train-script}
  \end{figure}
